Selection in Scientific Networks

One of the most interesting scientific challenges nowadays deals with the analysis and the understanding of complex networks' dynamics. A major issue is the definition of new frameworks for the exploration of the dynamics at play in real dynamic networks. Here, we focus on scientific communities by analyzing the "social part" of Science through a descriptive approach that aims at identifying the social determinants (e.g. goals and potential interactions among individuals) behind the emergence and the resilience of scientific communities. We consider that scientific communities are at the same time communities of practice (through co-authorship) and that they exist also as representations in the scientists' mind, since references to other scientists' works is not merely an objective link to a relevant work, but it reveals social objects that one manipulates and refers to. In this paper we identify the patterns about the evolution of a scientific field by analyzing a portion of the arXiv repository covering a period of 10 years of publications in physics. As a citation represents a deliberative selection related to the relevance of a work in its scientific domain, our analysis approaches the co-existence between co-authorship and citation behaviors in a community by focusing on the most proficient and cited authors interactions patterns. We focus in turn, on how these patterns are affected by the selection process of citations. Such a selection a) produces self-organization because it is played by a group of individuals which act, compete and collaborate in a common environment in order to advance Science and b) determines the success (emergence) of both topics and scientists working on them. The dataset is analyzed a) at a global level, e.g. the network evolution, b) at the meso-level, e.g. communities emergence, and c) at a micro-level, e.g. nodes' aggregation patterns.

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% "engineering"
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%

%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
% Non-BibTeX users please use
\begin{thebibliography}{99.}
%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references
%
% Monographs
\bibitem{monograph} Kipphan H (2000)
Handbook of printmedia. Springer, Berlin Heidelberg New York

% Contributed Works
\bibitem{contribution} Brandt J, Hein W (2001) Polymer materials in
joint surgery. In: Grellmann~W, Seidler S (eds)
Deformation and fracture behavior of polymers. Engineering
materials. Springer, Berlin Heidelberg New York

% Journal
\bibitem{journal} Che M, Grellmann W, Seidler S (1997)
Appl Polym Sci 64:1079--1090

% Theses
\bibitem{thesis} Ross DW (1977) Lysosomes and storage diseases. MA
Thesis, Columbia University, New York

\end{thebibliography}

